Drone-as-a-Service Composition Under Uncertainty

We propose an uncertainty-aware service approach to provide drone-based delivery services called Drone-as-a-Service (DaaS) effectively. Specifically, we propose a service model of DaaS based on the dynamic spatiotemporal features of drones and their in-flight contexts. The proposed DaaS service approach consists of three components: scheduling, route-planning, and composition. First, we develop a DaaS scheduling model to generate DaaS itineraries through a Skyway network. Second, we propose an uncertainty-aware DaaS route-planning algorithm that selects the optimal Skyways under weather uncertainties. Third, we develop two DaaS composition techniques to select an optimal DaaS composition at each station of the planned route. A spatiotemporal DaaS composer first selects the optimal DaaSs based on their spatiotemporal availability and drone capabilities. A predictive DaaS composer then utilises the outcome of the first composer to enable fast and accurate DaaS composition using several Machine Learning classification methods. We train the classifiers using a new set of spatiotemporal features which are in addition to other DaaS QoS properties. Our experiments results show the effectiveness and efficiency of the proposed approach.

==> R.tex <==
\setcounter{figure}{0}
\section*{Response}
We would like to extend our appreciation to the anonymous reviewers and associate editor. We believe their comments helped improve the quality and readability of the revised manuscript. Kindly find below our replies to the comments. \textit{Our replies are formatted in italic} and the \textbf{changes made in the paper are in bold}.

% \subsection*{General Note:}
% The current version has enhanced in terms of content and bibliography. The total word count has increased from 7,619 to 7,952 words. The bibliography references have increased from 31 to 32.

\subsection*{Associate Editor:}
\textit{We believe we have now addressed the reviewers' comments. We have coded the updates in the manuscript in bold and also copy the changes for each comment below.}

\subsection*{Reviewer: 1}
The paper is well-written and easy to follow in general. There are a few comments which must be addressed in order for this work to be published.

\textit{
Please find the response to this reviewer's  comments as follows:
}\newline

\begin{itemize}
    \item \underline{Comment:}
    \newline
    
    First, although uncertainty is highlighted in the title and the abstract, it’s not really paid much attention in the rest of the paper. Uncertainty is compensated only by adding or subtracting some uncertainty margin (CM) to the weather values, which are merely used as threshold to fly the drones or not. The value of CM is not even stated and its impacts are not analysed in the experiments.
    \newline
    
    \underline{Response:}
    \newline
    
    \textit{We revised the paper to highlight the focus on the uncertainty. We start the discussion about the uncertainty by the analysis given in the introduction. Then, we define a Certainty Margin (CM) as one standard deviation of the related measure, e.g, temperature, to be added or subtracted from the forecast measurement. This process aims to offer certain measurements to the DaaS route-planning algorithm to overcome the uncertainty problem. We have done statistical analyses on the historical weather data to show the variations between the predicted and actual measurements, as in Fig. \ref{actual-predicted} and Fig. \ref{actual-predicted-maps}.
    Then, we have investigated the impact of the uncertainty-aware A* against the greedy algorithm on the composed DaaS services, in Section \ref{ExpRes}, Tables \ref{tbl:heuristics} and \ref{heuristics}, and Fig. \ref{DaaS_resutls_error_rates}.
    We have finally focused on the uncertainty impacts in the results and discussion. We have now discussed the uncertainty in the problem definition, as follows (or on Page 3):}\newline
    \textbf{
    DaaS delivery service depends on weather conditions and regulations. 
    Fig. \ref{24_errors} shows an uncertainty analysis of multiple weather measurements. The blue-coloured horizontal line represents 0 deviations with the actual weather measurements. Fig. \ref{24_errors} illustrates that the uncertainty problem is affecting most of the weather measurements. For example, visibility forecast measurements are always higher than the actual measurements. We focus on the weather uncertainty; however, it can be found in other aspects such as uncertainty of package weights, battery levels and lifetime.}\newline
    
    
    \item \underline{New comment:}
    \newline
    \textcolor{red}{First, my previous concern on the “uncertainty” aspect is not really resolved. I am, of course, aware that there’s uncertainty in the weather data. But, the benefits of considering uncertainty is not shown with appropriate experiments. The authors’ response points to Tables 6 and 7, and Fig. 12. However, these merely shows that A* algorithms outputs something different from the Dijkstra algorithm. We could implement some different algorithm (which has nothing to do with uncertainty) and draw the same chart and tables to compare. For example, we could have an algorithm which minimizes the distance, not the skyway counts and draw the same graph, but this has nothing to do with uncertainty. 
    Can drones fail to deliver because uncertainty wasn’t considered in the Dijkstra algorithm? If so, it should be covered in the results section. 
    In addition, I am not sure of the purpose of having Fig. 12. Is it important whether the two algorithms output the same or different results? I would expect at least some results according to changing CM and show the delivery failure rates, etc.}
    
    \underline{New response:}
    \newline
    We have showed the impact of the uncertainty on the DaaS selections and the Machine learning classifiers performance. 
    A new subsection, (\ref{Error_Analysis} Error Analysis), is added to discuss the error analysis based on the CM impact. 
    We have rerun the whole experimental work on different CM values. Specifically, we have CM with values of: $1$, $2$, $3$, $4$, $5$, $10$, $15$, and $20$ standard deviation of the correspondent measure.
    Based on the reviewer suggestion, the experiments of these different Certainty Margins offers great insights to highlight the impact of the proposed uncertainty-aware DaaS composition algorithm.
    
    \textcolor{blue}{
    \subsection{Error Analysis}\label{Error_Analysis}
    In this section, we investigate the impact of using different CM values on the machine learning performance.
    We have selected the CM value to be a vector addition of two standard deviation ($CM2$) of the related measure, e.g., temperature. This selection is made based on the outcome of the error analysis on using different CM values such as one, two, three and more, as in Fig. \ref{CM_learning} and \ref{DaaS_resutls_error_rates}.
    Fig. \ref{CM_learning} shows the experimental results of using different CM values to compute the DaaS features for training the Logistic Regression classifier. Using the model with two standard deviations outperforms the other CMs. Using one standard deviation ($CM1$) comes in the second place with slightly decreased accuracy. Fig. \ref{CM_learning} shows the accuracy of using the $X4$ and $X5$ feature sets. It shows also a best-fit straight linear trend-line that describes the accuracy decreasing after the two standard deviation CM.
    Based on this outcome, we define the $CM2$ to be the best scheme in order to compare the different CM values. As using different CMs proves to have different learning performance, we investigate the CM impact on having wrong DaaS selections that have led to that accuracy decreasing. Fig. \ref{DaaS_resutls_error_rates} compares the different CMs to the $CM2$ in terms of their composite DaaS distance, duration, and length error. The $CM1$ has zero distance and length error while having 30.8\% error in the duration calculation in comparison to the behaviour of the the $CM2$. The error percentages of the three measures are steadily increasing when we increase the CM value. The $CM20$, for example, has $41.7\%$, $74.6\%$, and $32.1\%$ error selection for the distance, flying duration, and the DaaS length, in comparison to the $CM2$.
    We have also compared the utilisation of Dijkstra/A-star without the proposed heuristic algorithm. Fig. \ref{DaaS_resutls_error_rates} shows that Dijkstra has high error rates in comparison to the proposed heuristic A-star with the $CM2$.
    %
    \begin{figure}[!ht]
    \centering
    \includegraphics[width=0.60\textwidth]{Images/CM_LR.jpg}%\vspace{-1mm}
    \caption{The impact of using different CM values on the Logistic Regression classifier performance.}%\vspace{-4mm}
    \label{CM_learning}
    \end{figure}
    %
    %
    \begin{figure}[!ht]
    \centering
    \includegraphics[width=.60\textwidth]{Images/error_analysis.png}%\vspace{-4mm}
    \caption{Error percentages of using different CMs in comparison to the proposed $CM2$.}%\vspace{-4mm}
    \label{DaaS_resutls_error_rates}
    \end{figure}
    %
    }
    
    
    \item \underline{Comment:}
    \newline
    
    Second, the justifications for using the vast amount of weather related data such as including cloud coverage, temperature and humidity, seems to be a bit weak. What is the benefit of using dew point data instead of a more direct weather forecast such as “there will be a thunderstorm”. Is the 21C threshold for the dew point specific to the region or is it general enough to be applied in other areas? How does cloud coverage affect the flight duration? And how does an expert determine the threshold? How much does humidity impact the relative to temperature?
    \newline
    
    \underline{Response:}
    \newline
    
    \textit{Seeking for more accurate calculations, we utilise the weather measurements instead of the direct forecast. Specifically, we collect the weather measurements for the geo-location coordinates instead of general weather statuses. We define the utilised thresholds according to the aviation safety regulations and specialised experts online portals in weather forecast. We updated the text as follows  (or on Page 8):}\newline
    \textbf{
    We utilise the weather measurements instead of the direct forecast such as \textit{“there will be a thunderstorm”}. The purpose of this process is to produce for more accurate calculations. Specifically, we collect the weather measurements for the geo-location coordinates instead of general weather statuses. We define the above-mentioned thresholds according to the aviation safety regulations \footnote{These regulations are different from a country to another. In this research, we follow the regulations that are issued by the Civil Aviation Safety Authority (CASA).} and experts recommendations from online portals \footnote{we use recommendations from websites as the Aircraft Owners and Pilots Association (https://www.aopa.org/) and UAV Forecast (https://www.uavforecast.com/).}}
    \newline
    
    
    \item \underline{New comment:}
    \newline
    \textcolor{red}{More clarification is required for the second comment. The meaning of “more accurate calculations” is a bit vague. Is it more in line with the guidelines from uavforecast.com? or is the line 12 in Algorithm 1 results in exactly the same results as the website?}
    
    \underline{New response:}
    \newline
    We mean by the "More accurate calculations" is that the heuristic algorithm can used the quantitative measurements to select the optimal path. Having a useful direct weather status will not be the optimal information source as it would provided in limited complex situations. Instead of relying on qualitative weather statuses, it seems to be better using certain figures that can easily be compared against the utilised drones capabilities. Moreover, the proposed framework can simply modify the given measurements according to the employed drone. This flexibility makes the proposed approached independent to whatever drone type and flying environment. 
    We define the thresholds that used in Algorithm 1, line 12, according to the aviation safety regulations \footnote{These regulations are different from a country to another. In this research, we follow the regulations that are issued by the Civil Aviation Safety Authority (CASA).} and experts recommendations from online portals \footnote{we use recommendations from websites as the Aircraft Owners and Pilots Association (https://www.aopa.org/) and UAV Forecast (https://www.uavforecast.com/).}
    
    
    \textcolor{blue}{...}
    
    
    
    \item \underline{Comment:}
    \newline
    
     Third, does the framework assume that all DaaS for the future is known at the time of solving the composition problem? Is this realistic? Requests could arrive probabilistically real-time and this could be the most important source of uncertainty (more than weather data) when planning the schedules.\newline
     
    \underline{Response:}
    \newline
    
    \textit{Yes, the proposed framework consider the DaaS scheduling and planning problem. We assume that all the DaaS requests are known before. This is consistent with the the proposed delivery network. We design the use-case to have fixed delivery stations and DaaS requests. We have revised the text as follows (or on Page 1):}\newline
    \textbf{
    In the first component, we propose a new DaaS scheduling model that considers both cyber and physical processes. The proposed model constructs a delivery network that consists of delivery stations and sky-ways. We assume that all the DaaS requests are known before. We design the use-case to have fixed delivery stations and DaaS requests.}\newline
    
    \item \underline{New comment:}
    \newline
    \textcolor{red}{Regarding the third comment, I still cannot imagine an application where the DaaS requests are fixed. Could DaaS request be fixed and known ahead-of-time for lifesaving delivery or Google’s home delivery? I can easily assume home delivery requests will occur probabilistically, and they’d expect a short lead-time (30 minutes, otherwise why would you use drone delivery?). I do not think this is a killing comment, but I think the limits of the proposed algorithm should be clearly stated if this is the case.}
    
    \underline{New response:}
    \newline
    The proposed fixed DaaS delivery network have multiple potential applications. It is useful for a situation such as when a constructing company moves building materials and equipment among different work locations. They would have a prior plan of what to more and when. The plan can be considered to have multiple delivery requests in a sequence. This can be also applied in other examples such as mining companies, defence and border protections operations. Such domains may require moving reassures among different locations according to different planned schedules.  
    
    \textcolor{blue}{...}
    
    
    \item \underline{Comment:}
    \newline
    
    Fifth, how is crosswind taken into account? If there is significant crosswind, the drones will have to spend much more energy to stay on course, which means that it would consume much more energy to fly the same distance. It seems that only the head and tail wind is considered in equation (6)-(8). This could cause a major miscalculation about reachability of the drones to the destination?\newline
    
    \underline{Response:}
    \newline
    
    \textit{The cross wind calculation is explained in the Equation \ref{"Crosswind"}. However, it was mistakenly missed in the Equation \ref{"DAS"}. We have now updated the equation \ref{"DAS"} to express the cross wind as follows (or on Page 8):}\newline
    \textbf{
    Drone air speed (DAS) is computed as the subtraction of the GSA and WS.
    \begin{equation}\label{"DAS"}
        DAS = GSA \pm WS * \sin{(\theta)}
    \end{equation}
    The $\pm$ refers to the adding or subtracting the wind-speed in cases of tail or head wind types, respectively. The multiplication by $\sin{(\theta)}$ expresses the crosswind.}
    \newline
    
    \item \underline{New comment:}
    \newline
    \textcolor{red}{Regarding the fifth comment, I see that the drone power model is still wrong. I’d assume from Fig. 7, that theta=0 is headwind. (7) results in DAS=GSA for non-zero headwind (sin0 = 0). What I assume is that GSA is a fixed value for each drone. I think Windspeed + GSA should be a vector addition, and the direction of the resulting vector should be the same as the flight path. Depending on the direction of the sidewind, the direction of GSA should be different to fly to the destination.}
    
    \underline{New response:}
    \newline
    The drone power model is changed to be calculated on vector addition. The reviewer suggestion is better solving the problem specially in cases such what is provided in the reviewer's comment. 
    
    \textcolor{blue}{\textbf{
    Drone air speed (DAS) is computed as the subtraction of the GSA and WS.
    \begin{equation}\label{"DAS"}
        \Vec{DAS} = \Vec{GSA} + \Vec{WS}
    \end{equation}
    This vector addition refers to the adding or subtracting the wind-speed in cases of tail or head wind types.}}
    
    \item \underline{Comment:}
    \newline
    
     Sixth, I am wondering whether there was particular application that the authors had in mind. The number of nodes in the DaaS network graph seems to be quite small. If drones are carrying goods not only to major hubs but also to homes, etc., there would be a lot more number of nodes. Can the framework adapt to these scenarios?\newline
    
    \underline{Response:}
    \newline
    
    \textit{
    We considered the scenario where the delivery is done across fixed delivery stations and predefined sky-paths. This can be applied for e-commerce or governmental organisation. However, if we consider the ability of the proposed framework to plan an schedule DaaSs, this can be easily deployed in other use-cases such as home deliveries. We revised the text to make this information clear, as follows (or on page 3):}\newline
    \textbf{In this paper, we focus on the scenario of the delivery across fixed delivery stations and predefined sky-paths. This scenario can be applied for e-commerce or governmental organisation. However, our proposed framework can be deployed in other use-cases such as lifesaving delivery \footnote{flyzipline.com} and Google's home delivery \footnote{bbc.com/news/technology-47880288.}}\newline
    
    \item \underline{New comment:}
    \newline
    \textcolor{red}{My sixth comment was about the number of nodes. Google’s home delivery could result in hundreds of thousands of destination nodes. Would the algorithm be easily scalable?}
    
    \underline{New response:}
    \newline
    Yes, the proposed algorithm proved to be easily scalable. We have re-designed the DaaS delivery network to host $1,254$ nodes. We kept the old small network for scaling-comparison and visualisation purposes. 
    
    \textcolor{blue}{
    According to our delivery scenario, we construct a Skyways network that consists of $1,254$ delivery stations that are connected by $1,280$ Skyways.
    For simplicity, we discuss the uncertainty issues and DaaS composition on a small network of $38$ fixed delivery stations and $64$ Skyways.
    }
    \newline
    \textcolor{blue}{
    We generated small and large datasets using the above-mentioned DaaS delivery services scheduling and drone types. The large network has $1,254$ delivery stations as nodes, $1,280$ Skyways as edges, and the two drone types to define $16,770 $ DaaS delivery services. The small network has $38$ nodes and $64$ edges or Skyways with $30,476$ drone services. 
    Table \ref{DaaS-service} shows a sample of the generated DaaS dataset. For example, the DaaS number 1 flies from the source station \textit{E} to the destination \textit{A}. The total distance of the service flying is $169.19$ km consuming $197.6$ minutes of flying and maintenance over $16$ segments. The generated services are scheduled within two time ranges. First, it starts from 1st to the 9th of November, 2017. Second, it starts from 1st to the 9th of May, 2018. We simulated the movements of the generated services between the delivery stations. Table \ref{DaaS-simulation} lists the first movements of the DaaS with ID = 1. The total number of simulated movements is $4,589,290$ for the large network and $478,398$ for the small one. 
    Fig. \ref{DaaS_distribtions} highlights the distributions of the simulated services across the different delivery stations. It shows the closeness density of DaaSs at each delivery station. The dark-red colour represents service counts greater that $30,000$ and the dark-blue is for less than $5,000$. For example, Fig. \ref{DaaS_distribtions} shows that the delivery station \textit{E} hosts the largest number of services. This is due to the central location of \textit{E} that enables connecting such a large number of services. We used the \emph{darksky.net} API to collect the forecast weather measurements at the source and destination coordinates for each Skyway. We collected $1,294,185$ and $16,000$ records of the weather data within the predefined two time ranges for the two networks, i.e, large and small, respectively. The collected API data include various weather attributes such as temperature, cloud cover, wind speed, wind bearing, humidity, pressure, and dew-point. 
}
    
    \item \underline{Comment:}
    \newline
    
    Seventh, how realistic is the data generated from Section 5.3? Is there a particularly distribution, or assumptions for generating the data?
    
    \textit{Section \ref{Data-Collection} explains the generation of synthetic dataset for DaaS services schedules and requests. This dataset is generated based on the combination of the real weather data, real-coordinates for the delivery stations and sky-ways, and the real capabilities of drone models. The spatial distribution of the delivery stations is constrained by the CASA regulations as in Fig. \ref{DaaS_network_graph}. As a prototype design, we have also selected to make it far from the populous areas to avoid the privacy issues. We have updated the text in the discussion section as follow (or on Page 12):
    }\newline
    
    \underline{Response:}
    \newline
    \textbf{Here, we also notice that the generated DaaS services were successfully processed by the proposed DaaS framework. This dataset is generated based on the combination of the real weather data, real-coordinates for the delivery stations and sky-ways, and the real capabilities of drone models. The spatial distribution of the delivery stations is constrained by the CASA regulations as in Fig. \ref{DaaS_network_graph}. As a prototype design, we have also select to make it far from the populous areas to avoid the privacy issues.}\newline
    
    \item \underline{New comment:}
    \newline
    \textcolor{red}{Regarding seventh comment, I was more thinking of “DaaS request profiles” over time and space. For example, did the authors assume a uniform distribution over time? Because I don’t think there’s yet “real request” model.}
    
    \underline{New response:}
    \newline
    The generated DaaS requests are randomly distributed over time under normal (Gaussian) distribution.
    \textcolor{blue}{...}
    
\end{itemize}

\underline{Minor comments:}
\begin{itemize}
    \item In Fig. 12 caption, “powerful of the”\newline
    \item The text in the figures are too small to read. All should be reformatted.
    \item The captions in Fig. 14 and 15 are misleading. They don’t show “counts” but rather “distances”, don’t they? The units of the y-axes are (km). It’s also unclear what the graph above and below are different.
    \item Reference to Table 6 in “As listed in Table 6,” is wrong. I think it should refer to Table 7?
\end{itemize}

\subsection*{Reviewer: 2}
The manuscript is technically sound and proposes a good way of application of uncertainty methods and machine learning. The underlying uncertainty analysis makes this manuscript readable and relevant.
\newline
The title, the abstract and the keywords are chosen appropriately for this publication. The objectives of the manuscript are stated in the introduction in terms that encourage the reader to read on.
\newline
The manuscript is organized well, but could use a little bit more focus. The length is in deed appropriate for the topic and for presenting the ways of application. Most parts of the manuscript are easy to read, others need some effort to understand. All in all the manuscript is readable.
\newline
The manuscript can be published as is.
\newline
\textit{We thank the reviewer for his review.}

==> Response.tex <==
\setcounter{section}{0}
\setcounter{figure}{0}
\setcounter{table}{0}

\section*{Response}



Dear editor, 


We would like to thank the editor and all reviewers for their valuable comments and constructive feedback. We have carefully considered all the comments and made changes to the manuscript accordingly. In this response letter, we list the comments from the reviewers and our response to each comment.
 \textit{Our responses are formatted in italic} and the \textbf{changes made in the paper are in bold}.
 
 Best Regards,
 
 
 A. Hamdi, F. Salim, D.Y. Kim, A. Ghari Neiat, A. Bouguettaya



\subsection*{General Note:}
The current version has enhanced with major updates and revisions. One major update is that we re-scaled the network to have $1254$ nodes instead of only 38. This led to millions of DaaS selection. Accordingly, extensive experimental work had been done showing new interesting insights. We have also added a deep analysis of varying the certainty margin and its impact on the DaaS selection and machine learning performance. The impact of the proposed uncertainty DaaS composer is now better presented. New section and appendices are added to explain these new experiments and results. We have extended the discussion on the generated datasets presenting deep analyses and visualisations of different data distributions.


\subsection*{Reviewer: 1}
\textit{
Please find the response to this reviewer's comments as follows:
}\newline

\begin{itemize}
    \item \underline{Comment:}
    \newline
    First, my previous concern on the "uncertainty" aspect is not really resolved. I am, of course, aware that there's uncertainty in the weather data. But, the benefits of considering uncertainty is not shown with appropriate experiments. The authors' response points to Tables 6 and 7, and Fig. 12. However, these merely shows that A* algorithms outputs something different from the Dijkstra algorithm. We could implement some different algorithm (which has nothing to do with uncertainty) and draw the same chart and tables to compare. For example, we could have an algorithm which minimizes the distance, not the skyway counts and draw the same graph, but this has nothing to do with uncertainty. 
    Can drones fail to deliver because uncertainty wasn't considered in the Dijkstra algorithm? If so, it should be covered in the results section. 
    In addition, I am not sure of the purpose of having Fig. 12. Is it important whether the two algorithms output the same or different results? I would expect at least some results according to changing CM and show the delivery failure rates, etc.
    \newline
    \newline
    \underline{Response:}
    \newline
    \newline
    \textit{The package delivery is done through multiple drone-as-a-service (DaaS). Each DaaS flies from a source to a destination delivery stations. Dijkstra, or A* without the proposed heuristic method, produces incorrect delivery time estimations. We propose to utilise weather measurements to enable accurate heuristic-based path planning. However, the weather forecast measurements are uncertain. Our proposed method considers a Certainty Margin to fix this uncertainty issue. Based on the reviewer's suggestion, we have in-depth investigated the impact of the uncertainty on the DaaS selections and the Machine learning classifiers performance. 
    A new subsection, (9.3 Error Analysis), has been added to discuss the error analysis based on the CM impact. 
    We have rerun the whole experimental work on different CM values. Specifically, we have CM with values of: $1$, $2$, $3$, $4$, $5$, $10$, $15$, and $20$ standard deviation of the correspondent measure.
    The experiments of these different Certainty Margins offer excellent insights to highlight the impact of the proposed uncertainty-aware DaaS composition algorithm. We have updated as follows.}
    \newline
    \newline
    \textbf{
    9.3 Error Analysis. 
    In this section, we investigate the impact of using different CM values on machine learning performance.
    We have selected the CM value to be a vector addition of two standard deviations ($CM2$) of the related measure, e.g., temperature. This selection is made based on the outcome of the error analysis on using different CM values such as one, two, three and more, as shown in Fig. \ref{CM_learning} and \ref{DaaS_resutls_error_rates}.
    Fig. \ref{CM_learning} shows the experimental results of using different CM values to compute the DaaS features for training the Logistic Regression classifier. Using the model with two standard deviations outperforms the other CMs. Using one standard deviation ($CM1$) comes in second place with slightly decreased accuracy. Fig. \ref{CM_learning} shows the accuracy of using the $X4$ and $X5$ feature sets. It also shows a best-fit straight linear trend-line that describes the accuracy decreasing after the two standard deviation CM.
    Based on this outcome, we define the $CM2$ to be the best scheme in order to compare the different CM values. As using different CMs proves to have different learning performance, we investigate the CM impact on having wrong DaaS selections that have led to that accuracy decreasing. Fig. \ref{DaaS_resutls_error_rates} compares the different CMs to the $CM2$ in terms of their composite DaaS distance, duration, and length error. The $CM1$ has zero distance and length error while having 30.8\% error in the duration calculation in comparison to the behaviour of the $CM2$. The error percentages of the three measures are steadily increasing when we increase the CM value. The $CM20$, for example, has $41.7\%$, $74.6\%$, and $32.1\%$ error selection for the distance, flying duration, and the DaaS length, respectively, in comparison to the $CM2$.
    We have also compared the utilisation of Dijkstra/A-star without the proposed heuristic algorithm. Fig. \ref{DaaS_resutls_error_rates} shows that Dijkstra has high error rates in comparison to the proposed heuristic A-star with the $CM2$.
    %
    \begin{figure}[!ht]
    \centering
    \includegraphics[width=0.60\textwidth]{Images/CM_LR.jpg}%\vspace{-1mm}
    \caption{The impact of using different CM values on the Logistic Regression classifier performance.}%\vspace{-4mm}
    \label{CM_learning}
    \end{figure}
    %
    %
    \begin{figure}[!ht]
    \centering
    \includegraphics[width=.60\textwidth]{Images/error_analysis.png}%\vspace{-4mm}
    \caption{Error percentages of using different CMs in comparison to the proposed $CM2$.}%\vspace{-4mm}
    \label{DaaS_resutls_error_rates}
    \end{figure}
    %
    }
    \newline
    \newline
    \item \underline{Comment:}
    \newline
    More clarification is required for the second comment. The meaning of "more accurate calculations" is a bit vague. Is it more in line with the guidelines from uavforecast.com? or is the line 12 in Algorithm 1 results in exactly the same results as the website?
    \newline
    \newline
    \underline{Response:}
    \newline
    \newline
    \textit{The "More accurate calculations" means that the heuristic algorithm can use the quantitative measurements to select the optimal path. Having a direct weather status will not be the optimal information source as it would be provided in limited complex situations. Instead of relying on qualitative weather statuses, it seems to be better using certain figures that can easily be compared against the capabilities of the utilised drone. Moreover, the proposed framework can modify the given measurements according to the employed drone. This flexibility makes the proposed approaches independent of whatever drone type and flying environment. 
    We define the thresholds that used in Algorithm 1, line 12, according to the aviation safety regulations \footnote{These regulations are different from a country to another. In this research, we follow the regulations that are issued by the Civil Aviation Safety Authority (CASA).} and experts recommendations from online portals \footnote{we use recommendations from websites as the Aircraft Owners and Pilots Association (https://www.aopa.org/) and UAV Forecast (https://www.uavforecast.com/).}.
    These weather measurements prove to have clear impact on the performance of the machine learning classifiers as listed in Table 4 (on Page 12). We have added the subsection 9.2 as follows.
    }
    \newline
    \newline
    \textbf{9.2 Prediction Experimental Results
We generate a new dataset of $5,000$ PDRs to deliver packages among a number of sources and destinations around the delivery station \emph{E}. We choose \emph{E} because it is located in the centre of the network and has a large number of DaaS services, please refer to Fig. \ref{DaaS_distribtions}.
The generated DaaS requests are randomly distributed over time under normal (Gaussian) distribution.
We run the above-discussed components, as in Fig. \ref{DaaS-approach}, and collected the final selections by the \emph{spatiotemporal DaaS composer}. This process results in a large number of DaaS selections for the selected network stations.
\newline
The generated $5,000$ PDRs dataset results in $1,256,136$ and $25,676$ selections that are made by the \emph{spatiotemporal DaaS composer} using the large and small networks, respectively.
First, we utilised the small network to experiment with the different CM values. We then run the learning experiment on the large network with best CM value.
The selections are used as observations for cross-validation.  
We used the Python Scikit-learn package to implement the predictive DaaS composition models \cite{pedregosa2011scikit}. We trained four classifiers that represent different Machine Learning methods. The trained classifiers are Stochastic Gradient Descent (SGD), Support Vector Machine (SVM), Logistic Regression (LR), and Gaussian Naive Bayes (GNB).
Table \ref{tbl:ML_results} shows the results of the cross-validation using the feature sets from the large and small network, including $X1$, $X2$, $X3$, $X4$, and $X5$. $X1$ consists of the PDR features only. X2 combines the PDR and segments features. X3 adds the weather features to $X2$. $X4$ combines $X2$ with spatiotemporal features. Finally, X5 contains all four feature types. 
The weather properties improved the classification results as can be seen in the cases of $X3$ and $X5$. However, the new computed spatiotemporal features outperform the weather features. This is because the weather data are collected hourly while the spatiotemporal features are calculated for each timestamp at each delivery station. The small network based results show that using the \textbf{LR} classifier with the feature set $X5$ tend to the best performance with $99.84\%$ for $10-folds$ cross-validation using the $CM2$. However, the large network data lead to a more accurate selection of $99.89\%$.
    %
\begin{table*}[]
\caption{Evaluation of the proposed DaaS classification models using different feature sets.}\label{tbl:ML_results}
\begin{tabular}{|p{1.2cm}|l|l|l|l|l|l|l|l|l|p{1.2cm}|p{1.5cm}|p{1cm}|}
\hline
\multirow{2}{1cm}{Feature Set} &
  \multirow{2}{.5cm}{Model} &
  \multicolumn{8}{c|}{\begin{tabular}{c}\\Small Network (38 nodes)\end{tabular}} &
  Large Network (1254 nodes) &
  \multirow{2}{*}{Features} &
  \multirow{2}{0.6cm}{Feature count} \\ \cline{3-11}
 &
   &
  CM=1 &
  CM=2 &
  CM=3 &
  CM=4 &
  CM=5 &
  CM=10 &
  CM=15 &
  CM=20 &
  CM=2 &
   &
   \\ \hline
\multirow{4}{*}{X1} &
  SGD &
  37.56\% &
  38.50\% &
  37.17\% &
  35.10\% &
  33.62\% &
  33.58\% &
  33.56\% &
  37.28\% &
  41.26\% &
  \multirow{4}{*}{PDR} &
  \multirow{4}{*}{7} \\ \cline{2-11}
 &
  SVM &
  37.62\% &
  34.52\% &
  30.15\% &
  31.62\% &
  32.85\% &
  25.42\% &
  28.70\% &
  29.01\% &
  35.68\% &
   &
   \\ \cline{2-11}
 &
  LR &
  49.34\% &
  49.44\% &
  49.29\% &
  46.21\% &
  44.64\% &
  45.64\% &
  45.38\% &
  44.96\% &
  42.31\% &
   &
   \\ \cline{2-11}
 &
  GNB &
  51.23\% &
  50.68\% &
  50.08\% &
  43.33\% &
  41.57\% &
  40.44\% &
  38.61\% &
  39.81\% &
  44.9\% &
   &
   \\ \hline
\multirow{4}{*}{X2} &
  SGD &
  88.83\% &
  88.15\% &
  85.89\% &
  78.23\% &
  77.74\% &
  73.50\% &
  72.30\% &
  70.92\% &
  64.52\% &
  \multirow{4}{1.5cm}{PDR + segment} &
  \multirow{4}{*}{15} \\ \cline{2-11}
 &
  SVM &
  80.86\% &
  81.23\% &
  78.52\% &
  75.17\% &
  71.76\% &
  67.06\% &
  67.56\% &
  66.81\% &
  50.28\% &
   &
   \\ \cline{2-11}
 &
  LR &
  93.23\% &
  93.34\% &
  93.12\% &
  85.29\% &
  83.63\% &
  82.30\% &
  82.80\% &
  81.76\% &
  61.33\% &
   &
   \\ \cline{2-11}
 &
  GNB &
  95.82\% &
  95.83\% &
  95.21\% &
  88.30\% &
  84.93\% &
  83.39\% &
  80.35\% &
  79.82\% &
  84.54\% &
   &
   \\ \hline
\multirow{4}{*}{X3} &
  SGD &
  97.82\% &
  98.17\% &
  97.98\% &
  91.64\% &
  91.55\% &
  89.17\% &
  93.82\% &
  90.58\% &
  98.94\% &
  \multirow{4}{1.5cm}{PDR + segment + weather} &
  \multirow{4}{*}{17} \\ \cline{2-11}
 &
  SVM &
  97.12\% &
  95.77\% &
  97.22\% &
  90.47\% &
  90.44\% &
  87.02\% &
  90.68\% &
  90.65\% &
  97.66\% &
   &
   \\ \cline{2-11}
 &
  LR &
  98.81\% &
  98.92\% &
  99.09\% &
  94.54\% &
  94.24\% &
  91.68\% &
  93.94\% &
  94.18\% &
  99.6\% &
   &
   \\ \cline{2-11}
 &
  GNB &
  96.61\% &
  96.53\% &
  96.49\% &
  91.47\% &
  88.89\% &
  88.01\% &
  88.26\% &
  88.28\% &
  97.63\% &
   &
   \\ \hline
\multirow{4}{*}{X4} &
  SGD &
  94.23\% &
  94.49\% &
  94.15\% &
  83.14\% &
  86.40\% &
  80.76\% &
  82.09\% &
  82.56\% &
  86.19\% &
  \multirow{4}{1.7cm}{PDR + segment + spatiotemporal} &
  \multirow{4}{*}{11} \\ \cline{2-11}
 &
  SVM &
  89.45\% &
  84.50\% &
  89.49\% &
  83.56\% &
  80.60\% &
  79.73\% &
  78.11\% &
  79.67\% &
  83.62\% &
   &
   \\ \cline{2-11}
 &
  LR &
  96.05\% &
  96.15\% &
  95.77\% &
  89.85\% &
  88.38\% &
  88.54\% &
  89.49\% &
  89.24\% &
  85.32\% &
   &
   \\ \cline{2-11}
 &
  GNB &
  98.05\% &
  98.04\% &
  97.30\% &
  92.41\% &
  90.48\% &
  88.42\% &
  85.38\% &
  84.57\% &
  95.19\% &
   &
   \\ \hline
\multirow{4}{*}{X5} &
  SGD &
  98.39\% &
  98.72\% &
  98.46\% &
  91.98\% &
  92.11\% &
  94.10\% &
  94.19\% &
  93.42\% &
  99.71\% &
  \multirow{4}{1.9cm}{PDR + segment + spatiotemporal + weather} &
  \multirow{4}{*}{19} \\ \cline{2-11}
 &
  SVM &
  97.47\% &
  97.36\% &
  97.49\% &
  92.59\% &
  92.70\% &
  93.17\% &
  94.60\% &
  94.63\% &
  99.79\% &
   &
   \\ \cline{2-11}
 &
  \textbf{LR} &
  \textbf{99.74\%} &
  \textbf{99.84\%} &
  \textbf{99.68\%} &
  \textbf{95.72\%} &
  \textbf{95.75\%} &
  \textbf{95.83\%} &
  \textbf{96.02\%} &
  \textbf{95.95\%} &
  \textbf{99.89\%} &
   &
   \\ \cline{2-11}
 &
  GNB &
  97.15\% &
  97.15\% &
  96.90\% &
  93.05\% &
  90.68\% &
  89.55\% &
  89.94\% &
  90.24\% &
  98.42\% &
   &
   \\ \hline
\end{tabular}
\end{table*}
    }
\newline
    \newline
    \item \underline{Comment:}
    \newline
    \newline
     Regarding the third comment, I still cannot imagine an application where the DaaS requests are fixed. Could DaaS request be fixed and known ahead-of-time for lifesaving delivery or Google's home delivery? I can easily assume home delivery requests will occur probabilistically, and they'd expect a short lead-time (30 minutes, otherwise why would you use drone delivery?). I do not think this is a killing comment, but I think the limits of the proposed algorithm should be clearly stated if this is the case.
    \newline
    \newline
    \underline{Response:}
    \newline
    \newline
    \textit{The proposed fixed DaaS delivery network has multiple potential applications. It is useful for a situation such as when a constructing company moves building materials and equipment among different work locations. They would have a preliminary plan of what to more and when. The plan can be considered to have multiple delivery requests in a sequence. This can also be applied in other examples such as mining companies, defence and border protections operations. Such domains may require moving reassures among different locations according to different planned schedules. We have added the subsection (3.1 Problem Definition) as follows.}
    \newline
    \newline
    \textbf{In this paper, we focus on the scenario of the delivery across fixed delivery stations and predefined sky-paths. This scenario can be applied for e-commerce or governmental organisation. 
    It is useful for a situation such as when a constructing company moves building materials and equipment among different work locations. They would have a preliminary plan of what to more and when. The plan can be considered to have multiple delivery requests in a sequence. This can also be applied in other examples such as mining companies, defence and border protections operations. Such domains may require moving reassures among different locations according to different planned schedules. The proposed framework can also be deployed in other use-cases such as lifesaving delivery \footnote{flyzipline.com}.}
    \newline
    \newline
    \item \underline{Comment:}
    \newline
    Regarding the fifth comment, I see that the drone power model is still wrong. I'd assume from Fig. 7, that theta=0 is a headwind. (7) results in DAS=GSA for non-zero headwind (sin0 = 0). What I assume is that GSA is a fixed value for each drone. I think Windspeed + GSA should be a vector addition, and the direction of the resulting vector should be the same as the flight path. Depending on the direction of the sidewind, the direction of GSA should be different to fly to the destination.
    \newline
    \newline
    \underline{Response:}
    \newline
    \newline
    \textit{The drone power model is changed to be calculated on vector addition. The reviewer suggestion is better solving the problem, specially in cases such what is provided in the reviewer's comment.} 
    \newline
    \newline
    \textbf{
    Drone airspeed (DAS) is computed as the subtraction of the GSA and WS.
    \begin{equation}\label{"DAS"}
        \Vec{DAS} = \Vec{GSA} + \Vec{WS}
    \end{equation}
    This vector addition refers to the adding or subtracting the windspeed in cases of a tail or head wind types.}
    \newline
    \newline
    \item \underline{Comment:}
    \newline
    \newline
     My sixth comment was about the number of nodes. Google's home delivery could result in hundreds of thousands of destination nodes. Would the algorithm be easily scalable?
    \newline
    \newline
    \underline{Response:}
    \newline
    \newline
    \textit{Yes, the proposed algorithm proved to be easily scalable. To answer this question, we have re-designed the DaaS delivery network to host $1,254$ nodes instead of only $38$ in the previous submission. We kept the old small network for scaling-comparison and visualisation purposes. The paper is aupdated as follows:}
    \newline
    \newline
    \textbf{
    According to our delivery scenario, we construct a Skyways network that consists of $1,254$ delivery stations that are connected by $1,280$ Skyways.
    For simplicity, we discuss the uncertainty issues and DaaS composition on a small network of $38$ fixed delivery stations and $64$ Skyways.
    }
    \newline
    \newline
    \textbf{
    We generated small and large datasets using the above-mentioned DaaS delivery services scheduling and drone types. The large network has $1,254$ delivery stations as nodes, $1,280$ Skyways as edges, and the two drone types to define $16,770 $ DaaS delivery services. The small network has $38$ nodes and $64$ edges or Skyways with $30,476$ drone services. 
    Table \ref{DaaS-service} shows a sample of the generated DaaS dataset. For example, the DaaS number 1 flies from the source station \textit{E} to the destination \textit{A}. The total distance of the service flying is $169.19$ km, consuming $197.6$ minutes of flying and maintenance over $16$ segments. The generated services are scheduled within two-time ranges. First, it starts from 1st to the 9th of November, 2017. Second, it starts from 1st to the 9th of May, 2018. We simulated the movements of the generated services between the delivery stations. Table \ref{DaaS-simulation} lists the first movements of the DaaS with ID = 1. The total number of simulated movements is $4,589,290$ for the large network and $478,398$ for the small one. 
    Fig. \ref{DaaS_distribtions} highlights the distributions of the simulated services across the different delivery stations. It shows the closeness density of DaaSs at each delivery station. The dark-red colour represents service counts greater than $30,000$ and the dark-blue is for less than $5,000$. For example, Fig. \ref{DaaS_distribtions} shows that the delivery station \textit{E} hosts the largest number of services. This is due to the central location of \textit{E} that enables connecting such a large number of services. We used the \emph{darksky.net} API to collect the forecast weather measurements at the source and destination coordinates for each Skyway. We collected $1,294,185$ and $16,000$ records of the weather data within the predefined two time ranges for the two networks, i.e, large and small, respectively. The collected API data include various weather attributes such as temperature, cloud cover, wind speed, wind bearing, humidity, pressure, and dew-point. 
}
    \newline
    \newline
    \item \underline{Comment:}
    \newline
    \newline
    Regarding seventh comment, I was more thinking of "DaaS request profiles" over time and space. For example, did the authors assume a uniform distribution over time? Because I don't think there's yet "real request" model.
    \newline
    \newline
    \underline{Response:}
    \newline
    \newline
    \textit{The generated DaaS requests are uniformly distributed over time and locations under distribution. We have updated the Section (9.2 Prediction Experimental Results) and added a new Appendix to explain more details on the distributions of the generated datasets.}
    \newline
    \newline
    \textbf{Fig. \ref{PDR_dist2} highlights the DaaS delivery requests distributions. The delivery requests generated data show uni-from distribution over all the data attributes. The DaaS requests are symmetrically distributed over delivery weight, request time, geo-locations of source and destination, and pick-up time. More analyses on the generated data distributions are found in Appendix \ref{Appendix_data}.}
    %
    \begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.99\textwidth]{Images/PDR_distributions2.png}
    \caption{DaaS delivery requests show uni-from distribution over all the data attributes.}
    \label{PDR_dist2}
    \end{figure*}
    %
    \newline
    \newline
    \textbf{APPENDIX B DaaS Dataset
In this Appendix, we show more details about the generated DaaS dataset. We generate three main datasets for large and small scale network. 
\begin{itemize}
    \item First, DaaS Skyways network has $2,560$ and $128$ segment-connections between the network nodes for the large and small networks, respectively. Table \ref{network-Skyways} shows examples of the constructed Skyways.
    \item Second, DaaS services have $16,770$ and $30,476$ complete-paths that consist of several movements among the network station, for both the large and small networks, respectively. Table \ref{DaaS-service} lists samples of the DaaS services. These services refer to the virtual drones available at certain locations in particular timestamps. 
    \item Third, the later selections are in total of $4,589,290$ and $478,398$ DaaSs for the large and small delivery networks, respectively.
\end{itemize}
%
\begin{table}
%%\vspace{-2mm}
\centering
\caption{Examples of the constructed DaaS network Skyways.}%%\vspace{-3mm}
\label{network-Skyways}
\begin{tabular}{|p{0.5cm}|l|p{1cm}|p{2cm}|p{2cm}|p{2.5cm}|}
\hline
ID & Skyway       & Source & Desti-nation & Distance (km) & Compass bearing \\ \hline
1  & F-DS\_30      & F      & DS\_30      & 8.19     & 6                \\ \hline
2  & DS\_30-DS\_31 & DS\_30 & DS\_31      & 8.03     & 2                \\ \hline
3  & DS\_32-DS\_33 & DS\_32 & DS\_33      & 11.20    & 42               \\ \hline
4  & DS\_13-DS\_16 & DS\_13 & DS\_16      & 10.57    & 170              \\ \hline
5  & A-DS\_20      & A      & DS\_20      & 18.92    & 224              \\ \hline
6  & DS\_27-DS\_29 & DS\_27 & DS\_29      & 14.21    & 242              \\ \hline
7  & DS\_32-DS\_38 & DS\_32 & DS\_38      & 16.21    & 96               \\ \hline
8  & DS\_24-DS\_25 & DS\_24 & DS\_25      & 9.93     & 268              \\ \hline
9  & DS\_15-DS\_16 & DS\_15 & DS\_16      & 3.69     & 71               \\ \hline
10 & DS\_11-DS\_12 & DS\_11 & DS\_12      & 9.05     & 233              \\ \hline
\end{tabular}
\end{table}
%
\begin{table*}[h!]
\small
\centering
\caption{A sample of the generated DaaS delivery service dataset.}%\vspace{-5mm}
\label{DaaS-service}
\begin{tabular}{|l|l|l|p{1cm}|p{1cm}|p{1cm}|p{1.5cm}|p{1.2cm}|p{1cm}|p{5cm}|}
\hline
ID & Drone & Source & Desti. & Total distance & Flying Duration & Main-tenance time & Start time & Skyway count & stations \\ \hline
1 & M200 & E & A & 169.19 km & 122.6 min.& 75 min. & 11/1/17 1:00 & 16 & E-DS\_36-DS\_37-DS\_38-DS\_32-DS\_31-DS\_27-DS\_29-DS\_26-DS\_25-DS\_24-DS\_13-DS\_16-DS\_17-C-DS\_20-A \\ \hline
2 & M200 & E & A & 158.31 km & 114.7 min.& 70 min. & 11/1/17 1:00 & 15 & E-DS\_28-DS\_30-DS\_29-F-DS\_26-DS\_25-D-DS\_24-DS\_13-DS\_12-B-DS\_11-DS\_10-DS\_9-A \\ \hline
\end{tabular}
\end{table*}
%
\begin{table}[h!]
\centering
\caption{DaaS delivery services movements.}
\label{DaaS-simulation}
% \small
\begin{tabular}{|p{0.5cm}|p{2cm}|p{2.5cm}|p{1.5cm}|p{2.4cm}|p{2.2cm}|p{2cm}|}
\hline
ID & Flying duration & \makecell{Arrival\\ time} & Sou-rce & Desti-nation & Skyway number & Total Skyways \\ \hline
1 & 2.7 & 2017-11-01 01:02:45 & E & DS\_36 & 1 & 16 \\ \hline
1 & 2.2 & 2017-11-01 01:20:01 & DS\_36 & DS\_37 & 2 & 16 \\ \hline
1 & 4.6 & 2017-11-01 01:39:37 & DS\_37 & DS\_38 & 3 & 16 \\ \hline
1 & 11.7 & 2017-11-01 02:06:22 & DS\_38 & DS\_32 & 4 & 16 \\ \hline
1 & 6.0 & 2017-11-01 02:27:22 & DS\_32 & DS\_31 & 5 & 16 \\ \hline
1 & 13.2 & 2017-11-01 02:55:34 & DS\_31 & DS\_27 & 6 & 16 \\ \hline
1 & 10.2 & 2017-11-01 03:20:52 & DS\_27 & DS\_29 & 7 & 16 \\ \hline
\end{tabular}
\end{table}
%
Fig. \ref{Seg_dist} shows DaaS Skyways (segments) has different distributions in terms of different attributes such as geo-location longitude and latitude of source and destination stations, and compass-bearing direction of the segment. Both the large and small network have normal (symmetrical) distributions are symmetrically or equally distributed across the mean. However, the two networks have different distribution-modes. The small network mostly has bimodal uniform distribution, and the large one has multi-modal ones. These Multi-modal distributions are combining multiple distribution modes around different geo-locations. 
\newline
Fig \ref{Ser_dis} shows DaaS services' distributions of different attributes such as distance, flying duration, handling time, and DaaS start time. The Figure has four columns of graphs visualising (from left to right): 
1) distribution with mean and standard deviation on the large network,
2) distribution with data percentile on the large network,
3) distribution with mean and standard deviation on the small network, and
4) distribution with data percentile on the small network.
Generally, the graphs are not perfectly symmetric, but they show uniform distribution around the mean.
In terms of segment count, the distribution graphs are left-skewed (negative-skewed) having bells at high counts (right-side) with tails at low segment counts. This insight shows that high counts of selection are frequently found in the composite DaaS.
\newline
Fig. \ref{PDR_dist} highlights the DaaS delivery requests distributions. The generated data of request show uniform distribution over all the data attributes. The DaaS requests are symmetrically distributed over delivery weight, request time, geo-locations of source and destination, and pick-up time.
%
\begin{figure*}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{Images/DaaS_Segments_distributions}
\caption{DaaS Skyways (segments) has different distributions in terms of different attributes such as geo-location longitude and latitude of source and destination stations, and compass-bearing direction of the segment.}
\label{Seg_dist}
\end{figure*}
%
\begin{figure*}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{Images/DaaS_Services_distributions}
\caption{DaaS services' distributions of different attributes such as distance, flying duration, handling time, and DaaS start time. The Figure has four columns of graphs visualising (from left to right): 
1) distribution with mean and standard deviation on the large network,
2) distribution with data percentile on the large network,
3) distribution with mean and standard deviation on the small network, and
4) distribution with data percentile on the small network.}
\label{Ser_dis}
\end{figure*}
%
\begin{figure*}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{Images/PDR_distributions.png}
\caption{DaaS delivery requests show uniform distribution over all the data attributes.}
\label{PDR_dist}
\end{figure*}
%
}
\end{itemize}

\clearpage
\underline{Minor comments:}
\newline
\begin{itemize}
    \item In Fig. 12 caption, “powerful of the” $\leftarrow$ Corrected. 
    \newline
    \item The text in the figures are too small to read. All should be reformatted. $\leftarrow$ Updated.
    \newline
    \item The captions in Fig. 14 and 15 are misleading. They don't show "counts" but rather "distances", don't they? The units of the y-axes are (km). It's also unclear what the graph above and below are different. $\leftarrow$ Updated.
    \newline
    \item Reference to Table 6 in "As listed in Table 6," is wrong. I think it should refer to Table 7? $\leftarrow$ Corrected.
\end{itemize}

\subsection*{Reviewer: 2}
The manuscript is technically sound and proposes a good way of application of uncertainty methods and machine learning. The underlying uncertainty analysis makes this manuscript readable and relevant.
\newline
The title, the abstract and the keywords are chosen appropriately for this publication. The objectives of the manuscript are stated in the introduction in terms that encourage the reader to read on.
\newline
The manuscript is organized well, but could use a little bit more focus. The length is in deed appropriate for the topic and for presenting the ways of application. Most parts of the manuscript are easy to read, others need some effort to understand. All in all the manuscript is readable.
\newline
The manuscript can be published as is.
\newline\newline
\textit{We have revised the paper adding more details on the DaaS algorithm, generated datasets, and the machine learning performance. We have also added new appendices to provide more discussion on these sections.}
